SplitFS: Reducing Software Overhead in File Systems for Persistent Memory

We present SplitFS, a file system for persistent memory (PM) that reduces software overhead significantly compared to state-of-the-art PM file systems. SplitFS presents a novel split of responsibilities between a user-space library file system and an existing kernel PM file system. The user-space library file system handles data operations by intercepting POSIX calls, memory-mapping the underlying file, and serving the read and overwrites using processor loads and stores. Metadata operations are handled by the kernel PM file system (ext4 DAX). SplitFS introduces a new primitive termed relink to efficiently support file appends and atomic data operations. SplitFS provides three consistency modes, which different applications can choose from, without interfering with each other. SplitFS reduces software overhead by up-to 4x compared to the NOVA PM file system, and 17x compared to ext4-DAX. On a number of micro-benchmarks and applications such as the LevelDB key-value store running the YCSB benchmark, SplitFS increases application performance by up to 2x compared to ext4 DAX and NOVA while providing similar consistency guarantees.

==> fig-bkgd.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{Figures/sosp_bkgd_crop.pdf}
\mycaption{Persistent memory system}{The figure shows
  how persistent memory will be placed alongside DRAM in the memory
  hierarchy, along with empirically measured latencies for different
  methods to write to persistent memory. Writes become persistent once
  they reach the persistent-memory controller. Writes can be made
  persistent either using non-temporal stores instructions or temporal
  store and cache line flush instrucions.}
\label{fig-bkgd}
\vspace{-10pt}
\end{figure}


==> fig-mot.tex <==
\begin{figure}
\centering \includegraphics[width=0.48\textwidth]{graphs/mot.png}
\mycaption{Write Latency}{The figure shows the average latency of a
  POSIX \syswrite call (writing 4KB in an existing file) on various
  PM file systems, and on the raw device itself. The
  overhead shown in parenthesis is the ratio of \syswrite latency to
  PM device write latency.}

\label{fig-mot}
\end{figure}


==> fig-sw-ovhd-micro.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{Figures/ledger-sw-micro.png}
\mycaption{microbench SW overhead}{}
\label{fig-factor}
\vspace{-10pt}
\end{figure}


==> panda-pm.tex <==
\section{Methodology}
\label{sec-methodology}

In this section, we will talk about the procedure that is used to check crash consistency of persistent memory file systems. We first talk about the platform that we use in order to track memory writes, cacheline flushes and memory fence instructions (\sref{sec-panda}) and then we talk about how this information is used to check the crash consistency in file systems (\sref{sec-crashmonkey-panda}).

\subsection{PANDA}
\label{sec-panda}

Panda is a dynamic execution engine based on QEMU. When a basic block of code is executed in the guest, the QEMU virtual machine monitor converts the block of guest code into an intermediate language. From this intermediate language, QEMU generates a binary code block which is directly executed on the host, in order to emulate the guest code block. Panda analyzes the intermediate language generated by QEMU for specific instructions of interest. With Panda, users are allowed to track memory loads and stores as well as flushes at specific address ranges through user defined plugins. Based on the tracked instructions, panda allows users register callback functions for logging the recorded data in a file, or performing some other tasks. The user defined plugins in Panda can be loaded arbitrarily when the user wants to track memory loads, stores and flushes, and they can be unloaded when the user is no longer interested in tracking instructions.

\subsection{CrashMonkey with PANDA}
\label{sec-crashmonkey-panda}

The procedure for checking crash consistency for persistent memory file systems is different for persistent memory than for disk based file systems, due to the differences mentioned in \sref{sec-complexities}. This subsection contains the steps that are used for testing crash consistency for persistent memory file systems.

\vheading{Initialization}. Since PANDA works in conjunction with QEMU and tracks memory accesses in the QEMU guest, a virtual machine is booted up with PANDA enabled, and with two memory regions reserved for persistent memory (pmem0 and pmem1). One of the memory regions (pmem0) is treated as a record device, and the second region (pmem1) is treated as a replay device.

\vheading{Snapshotting}. In this stage, an empty file system is created and mounted in the record device. This step performs file system initializations on the record device such as initializing the superblock and various other metadata structures of the file system. After the file system is created and mounted, a snapshot of the record device is taken and is restored on the replay device. This step does the file system initialization task at the replay device, but does not actually mount the file system.

\vheading{Tracing}. The PANDA plugin for tracking memory writes, memory fences and cacheline flushes is loaded for the region of memory that belongs to the record device. On loading the plugin, PANDA starts to analyze the intermediate language of QEMU for the store, fence and flush instructions. Callbacks are issued for each of these instructions to log them in a file. Now the workload to be tested is run on the record device. After the workload is completely executed, the PANDA plugin is unloaded in order to stop the tracking of instructions.

\vheading{Generation of crash states}. The log file is parsed and different crash states are generated by crashmonkey, in the same way as they are generated for disk based file systems.

\vheading{Checking crash recovery}. The different crash states are replayed at the replay device. After each crash state, the file system at the replay device is mounted to check if it recovers to a consistent state, and a bug report is generated if the file system fails to do so. 


==> tbl-apps.tex <==
\begin{table*}[!t]
  \small
  \centering
  \ra{1.3}
  \begin{tabular}{@{}ll||p{25pt}p{25pt}p{25pt}p{25pt}p{25pt}p{25pt}p{25pt}p{25pt}p{25pt}p{25pt}||p{25pt}p{25pt}p{25pt}@{}}
    \toprule[1.2pt]
    \multicolumn{2}{c}{Config} & \multicolumn{10}{c}{Throughput Apps (KOps/s)} & \multicolumn{3}{c}{Latency Apps (sec)} \\
    \midrule
    Mode & System & Redis & TPCC & LoadA & LoadE & RunA & RunB & RunC & RunD & RunE & RunF & Tar & Git & Rsync \\
    \midrule
    POSIX & ext4-DAX & 83.56 & 5.41 & 30.84 & 30.69 & 72.64 & 146.28 & 191.93 & 214.92 & 15.24 & 122.72 & 32.53 & 29.41 & 15.01 \\
    POSIX & \sysname & 1.23x & 1.14x & 1.45x & 1.47x & 1.51x & 0.92x & 0.94x & 0.92x & 0.92x & 1.19x & 1.02x &1.10x & 0.98x\\
    \midrule
    Sync & PMFS & 102.99 & 6.17 & 44.84 & 44.99 & 109.88 & 134.99 & 181.12 & 196.76 & 13.99 & 145.47 & 32.9 & 27.81 & 13.63 \\
    %Sync & PMFS & 1.18x & 1.00x & 1.24x & 1.26x & 1.23x & 0.95x & 0.93x & 0.94x & 0.92x & 1.11x & 1.01x & 0.95x &0.91x\\
    %Sync & NOVA & 1.04x & 0.82x & 1.14x & 1.15x & 1.12x & 0.96x & 0.96x & 0.96x & 0.97x & 1.04x & 0.99x & 0.96x & 0.94x\\
    Sync & \sysname & 1.03 & 1.15 & 1.14 & 1.12 & 1.19 & 0.97 & 1.03 & 0.97 & 0.99 & 1.04 & 1.01 & 1.18 & 1.09 \\
    %Sync & \sysname & 1.21x  & 1.15x  & 1.42x & 1.40x & 1.46x & 0.92x & 0.96x & 0.91x  &  0.91x & 1.16x & 1.02x & 1.11x & 0.99x\\
    \midrule
    Sync & NOVA & 83.28 & 4.29 & 35.48 & 35.25 & 83.27 & 138.88 & 181.71 & 204.02 & 14.74 & 126.43 & 32.19 & 28.25 & 14.02 \\
    %Strict & NOVA & 1.00x & 0.79x & 1.15x & 1.15x & 1.15x & 0.95x & 0.95x & 0.95x & 0.97x & 1.03x & 0.99x & 0.96x &0.93x\\
    Strict & \sysname & 1.20 & 1.12 & 1.23 & 1.22 & 1.23 & 0.97 & 1.00 & 0.95 & 0.94 & 1.10 & 1.02 & 1.15 & 1.05x \\ 
    %Strict & \sysname & 1.20x & 0.89x & 1.41x & 1.40x & 1.41x & 0.92x & 0.95x & 0.90x & 0.91x & 1.13x & 1.01x & 1.10x & 0.98x\\
    \bottomrule[1.2pt]
  \end{tabular}
  \caption{Application performance table. \todo{PMFS numbers are wrong, but, \sysname (sync) numbers are correct.} \todo{Need to split this table, separate for throughtput and latency.}}
  \label{tbl-apps}
\end{table*}


==> tbl-comp.tex <==
\begin{table}[!t]
  \small
  \centering
  %\ra{1.3}
  \begin{tabular}{@{}p{92pt}ccccc@{}}
%\begin{tabularx}{50pt}{@{}lrp{2cm}@{}}    
    \toprule[1.2pt]
    File System & O & WA & C & R & P \\
    \midrule
    \emph{Ideal PM File System} & \gl & \gl & \gh & \gl & \gh \\
    \midrule
    PMFS & \badh & \gl & \ormed & \gl & \badl \\
    NOVA & \badh & \gl & \gh & \gl & \badl \\
    Strata & \gl & \ormed & \gh & \ormed & \ormed \\
    ext4 Direct Access (DAX) & \badh & \gl & \badl & \gl & \gh \\
    \midrule
    \sysname on ext4 DAX & \gl & \gl & \gh & \ormed & \gh \\
    \bottomrule[1.2pt]
   %\end{tabularx}
  \end{tabular}
  \vspace{5pt}
  \mycaption{Properties of PM File Systems}{The table
    compares properties of PM file systems to the ideal PM
    file system. Legend: O - Software overhead, WA - Write
    amplification, C - Consistency, R - Recovery time, P -
    Portability. The ideal value for each property is italicized and
    shown in green.  }
  \label{tbl-comp}
  \vspace{-15pt}
\end{table}


==> tbl-modes.tex <==
\begin{table}[!t]
  \small
  \centering
  %\ra{1.3}
  \begin{tabular}{@{}p{30pt}p{120pt}p{60pt}@{}}
%\begin{tabularx}{50pt}{@{}lrp{2cm}@{}}    
    \toprule[1.2pt]
    \emph{Mode} & \emph{Guarantees} & \emph{Equivalent to}\\
    \midrule
    POSIX & Synchronous data operations & ext4 DAX \\
    \midrule
    sync & Synchronous data and metadata operations & NOVA-Relaxed,
    PMFS \\
    \midrule
    strict & Synchronous, atomic data and metadata operations &
    NOVA-Strict, Strata \\
    \bottomrule[1.2pt]
   %\end{tabularx}
  \end{tabular}
  \vspace{5pt} \mycaption{\sysname modes}{The table shows the three
    modes that \sysname can be run in, the guarantees provided by each
    mode, and list current file systems which provide the same
    guarantees. %All modes ensure consistency of file-system metadata.
  }
  \label{tbl-modes}
  %\vspace{-15pt}
\end{table}


==> tbl-syscall-overhead.tex <==
\begin{table}[!t]
  %\small
  \centering
  \ra{1.3}
  %\begin{tabular}{@{}p{92pt}r@{}}
  \begin{tabular}{@{}llrrr@{}}
%\begin{tabularx}{50pt}{@{}lrp{2cm}@{}}    
    \toprule[1.2pt]
    Mode & System & LoadA & RunA & TPCC\\
    \midrule
    POSIX & \extdax & 3.29\myx & 2.80\myx & 1.79\myx \\
    \midrule
    Sync & PMFS & 1.45\myx & 1.29\myx & 1.77\myx \\
    Sync & NOVA & 2.24\myx & 2.09\myx & 3.79\myx \\
    \midrule
    Strict & NOVA & 2.21\myx & 2.12\myx & 1.37\myx \\
    \bottomrule[1.2pt]
   %\end{tabularx}
  \end{tabular}
  \vspace{5pt} \mycaption{File system software overheads}{For three different
  workloads, this table shows the relative software overheads
  suffered by different file systems compared to \sysname providing
  the same guarantees. We define software overhead as the time 
  consumed by system calls minus the time actually spent accessing PM.
  For example, if a write system call takes 100~\mus out of which only 25us
  were spent writing to PM, the software overhead is 75us (100-25).}
  \label{tbl-syscall-overhead}
  %\vspace{-20pt}
\end{table}


==> tbl-techniques.tex <==
\begin{table*}[!t]
  \small
  \centering
  %\ra{1.3}
  \begin{tabular}{@{}p{92pt}ccccc@{}}
%\begin{tabularx}{50pt}{@{}lrp{2cm}@{}}    
    \toprule[1.2pt]
    File System & O & WA & C & R & P \\
    \midrule
    \emph{Ideal PM File System} & \gl & \gl & \gh & \gl & \gh \\
    \midrule
    PMFS & \badh & \gl & \ormed & \gl & \badl \\
    NOVA & \badh & \gl & \gh & \gl & \badl \\
    Strata & \gl & \ormed & \gh & \ormed & \ormed \\
    ext4 Direct Access (DAX) & \badh & \gl & \badl & \gl & \gh \\
    \midrule
    \sysname on ext4 DAX & \gl & \gl & \gh & \ormed & \gh \\
    \bottomrule[1.2pt]
   %\end{tabularx}
  \end{tabular}
  \vspace{5pt}
  \mycaption{Properties of PM File Systems}{The table
    compares properties of PM file systems to the ideal PM
    file system. Legend: O - Software overhead, WA - Write
    amplification, C - Consistency, R - Recovery time, P -
    Portability. The ideal value for each property is italicized and
    shown in green.  }
  \label{tbl-comp}
  \vspace{-15pt}
\end{table*}


==> tbl-write-amp.tex <==
\begin{table}[!t]
  %\small
  \centering
  \ra{1.3}
  %\begin{tabular}{@{}p{92pt}r@{}}
  \begin{tabular}{@{}lrrrr@{}}
%\begin{tabularx}{50pt}{@{}lrp{2cm}@{}}    
    \toprule[1.2pt]
    System & Seq. & Rand. & Appends & Overwrites \\
    \midrule
    Strata & 2.1GB & 2.1GB & 2.2GB & 1.1GB \\
    \Sysname (strict)& 1.05GB & 1.05GB & 1.1GB & 1.05GB \\
    \bottomrule[1.2pt]
   %\end{tabularx}
  \end{tabular}
  \vspace{5pt} \mycaption{Low write amplification}{This table
  shows the amount of data actually written to PM when an applcation 
  performs 1GB worth os 4KB writes to a file along different patterns.}
  \label{tbl-write-amp}
\end{table}


==> tbl-ycsb-desc.tex <==
\begin{table}[!t]
  \small
  \centering
  \ra{1}
  \setlength\tabcolsep{6pt}
  \begin{tabular}{@{}p{1.2cm}p{3.2cm}p{3.2cm}@{}}
    \toprule[1.2pt]
    \textit{\textbf{Workload}} & \textit{\textbf{Description}}  &
    \textit{\textbf{Represents}}          \\
    \midrule
    Load A & 100\% writes & Insert data for workloads A--D and F \\
    \hline
    A                          & 50\% reads, 50\% writes        &
    Session recording recent actions      \\
        \hline

    B                          & 95\% reads, 5\% writes         &
    Browsing and tagging photo album      \\
        \hline

    C                          & 100\% reads                    &
    Caches                                \\
    \hline

    D                          & 95\% reads (latest values), 5\% writes    & News
    feed or status feed              \\
    \hline
    Load E & 100\% writes & Insert data for Workload E \\
    \hline

    E                          & 95\% Range queries, 5\% writes &
    Threaded conversation \\
    \hline

    F                          & 50\% reads, 50\% Read-modify-writes       &
    Database workload \\
    \bottomrule[1.2pt]
  \end{tabular}
  \vspace{1pt}
  \mycaption{YCSB Workloads}{The table describes the six
    workloads in the YCSB suite. Workloads A--D and F are preceded by
    Load A, while E is preceded by Load E. \ak{Maybe remove for space.}}
  \label{tbl-ycsb-desc}
  \vspace{-0.2in}
\end{table}

